Learning Feature Aggregation for Deep 3D Morphable Models

3D morphable models are widely used for the shape representation of an object class in computer vision and graphics applications. In this work, we focus on deep 3D morphable models that directly apply deep learning on 3D mesh data with a hierarchical structure to capture information at multiple scales. While great efforts have been made to design the convolution operator, how to best aggregate vertex features across hierarchical levels deserves further attention. In contrast to resorting to mesh decimation, we propose an attention based module to learn mapping matrices for better feature aggregation across hierarchical levels. Specifically, the mapping matrices are generated by a compatibility function of the keys and queries. The keys and queries are trainable variables, learned by optimizing the target objective, and shared by all data samples of the same object class. Our proposed module can be used as a train-only drop-in replacement for the feature aggregation in existing architectures for both downsampling and upsampling. Our experiments show that through the end-to-end training of the mapping matrices, we achieve state-of-the-art results on a variety of 3D shape datasets in comparison to existing morphable models.

==> tables/table_extrapolation_temperature_softmax.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table*}
\begin{center}
\caption{Reconstruction errors on extrapolation setting}
\label{table_extrapolation}
\begin{tabular}{l|cc|cc|cc|cc}
 & \multicolumn{2}{c|}{Deep3DMM(spectral)}	& \multicolumn{2}{c|}{CoMA~\cite{DBLP:conf/eccv/RanjanBSB18}}	& \multicolumn{2}{c|}{PCA} & \multicolumn{2}{c}{FLAME~\cite{DBLP:journals/tog/LiBBL017}} \\
Sequence & Mean Error & Median  & Mean Error & Median  & Mean Error & Median  & Mean Error & Median \\\hline
bareteeth  & \textbf{1.167$\pm$1.507} & \textbf{0.655}   & 1.376$\pm$1.536 & 0.856    & 1.957$\pm$1.888 & 1.335       & 2.002$\pm$1.456 & 1.606 \\
cheeks in  & \textbf{1.135$\pm$1.455} & \textbf{0.645}   & 1.288$\pm$1.501 & 0.794    & 1.854$\pm$1.906 & 1.179       & 2.011$\pm$1.468 & 1.609 \\
eyebrow  & \textbf{0.831$\pm$0.888} & \textbf{0.535}   & 1.053$\pm$1.088 & 0.706    & 1.609$\pm$1.535 & 1.090       & 1.862$\pm$1.342 & 1.516 \\
high smile  & \textbf{1.092$\pm$1.222} & \textbf{0.670}   & 1.205$\pm$1.252 & 0.772    & 1.841$\pm$1.831 & 1.246       & 1.960$\pm$1.370 & 1.625 \\
lips back  & \textbf{0.949$\pm$1.327} & \textbf{0.528}   & 1.193$\pm$1.476 & 0.708    & 1.842$\pm$1.947 & 1.198       & 2.047$\pm$1.485 & 1.639 \\
lips up  & \textbf{0.895$\pm$1.120} & \textbf{0.503}   & 1.081$\pm$1.192 & 0.656    & 1.788$\pm$1.764 & 1.216       & 1.983$\pm$1.427 & 1.616 \\
mouth down  & \textbf{0.811$\pm$0.998} & \textbf{0.504}   & 1.050$\pm$1.183 & 0.654    & 1.618$\pm$1.594 & 1.105       & 2.029$\pm$1.454 & 1.651 \\
mouth extreme  & \textbf{1.153$\pm$1.582} & \textbf{0.633}   & 1.336$\pm$1.820 & 0.738    & 2.011$\pm$2.405 & 1.224       & 2.028$\pm$1.464 & 1.613 \\
mouth middle  & \textbf{0.720$\pm$0.914} & \textbf{0.428}   & 1.017$\pm$1.192 & 0.610    & 1.697$\pm$1.715 & 1.133       & 2.043$\pm$1.496 & 1.620 \\
mouth open  & \textbf{0.774}$\pm$1.172 & \textbf{0.422}   & 0.961$\pm$\textbf{1.127} & 0.583    & 1.612$\pm$1.728 & 1.060       & 1.894$\pm$1.433 & 1.544 \\
mouth side  & \textbf{1.130}$\pm$1.766 & \textbf{0.578}   & 1.264$\pm$\textbf{1.611} & 0.730    & 1.894$\pm$2.274 & 1.132       & 2.090$\pm$1.510 & 1.659 \\
mouth up  & \textbf{0.833$\pm$0.971} & \textbf{0.495}   & 1.097$\pm$1.212 & 0.683    & 1.710$\pm$1.680 & 1.159       & 2.067$\pm$1.485 & 1.680 \\
\end{tabular}
\end{center}
\end{table*}


==> tables/table_filter.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{Reconstruction errors with different setting of filters }
\label{table_filter}
\begin{tabular}{lcc}
method      & simple    & wider    \\\hline
CoMA      & 0.939 & 0.682         \\ 
CoMA+FA   & 0.519     & 0.441     \\ \hline
Neural3DMM      & 0.785 & 0.525         \\ 
Neural3DMM+FA   & 0.487     & 0.420
\end{tabular}
\end{center}
\end{table}
